Co-op: Correspondence-based Novel Object Pose Estimation

We propose Co-op, a novel method for accurately and robustly estimating the 6DoF pose of objects unseen during training from a single RGB image. Our method requires only the CAD model of the target object and can precisely estimate its pose without any additional fine-tuning. While existing model-based methods suffer from inefficiency due to using a large number of templates, our method enables fast and accurate estimation with a small number of templates. This improvement is achieved by finding semi-dense correspondences between the input image and the pre-rendered templates. Our method achieves strong generalization performance by leveraging a hybrid representation that combines patch-level classification and offset regression. Additionally, our pose refinement model estimates probabilistic flow between the input image and the rendered image, refining the initial estimate to an accurate pose using a differentiable PnP layer. We demonstrate that our method not only estimates object poses rapidly but also outperforms existing methods by a large margin on the seven core datasets of the BOP Challenge, achieving state-of-the-art accuracy.

==> sec/figures/main_large.tex <==
\begin{center}
	\centering
	\includegraphics[width=\linewidth]{figures/main_figure.png}

	\captionof{figure}{Examples of 6D pose estimation of novel objects. Our method estimates correspondences between the input image and rendered image, and 6D object pose.}
	\label{fig:main}
\end{center}
